Shuffling the Data, Stretching the Step-size: Sharper Bias in constant step-size SGD

From adversarial robustness to multi-agent learning, many machine learning tasks can be cast as finite-sum min-max optimization or, more generally, as variational inequality problems (VIPs). Owing to their simplicity and scalability, stochastic gradient methods with constant step size are widely used, despite the fact that they converge only up to a constant term. Among the many heuristics adopted in practice, two classical techniques have recently attracted attention to mitigate this issue: \emph{Random Reshuffling} of data and \emph{Richardson--Romberg extrapolation} across iterates. Random Reshuffling sharpens the mean-squared error (MSE) of the estimated solution, while Richardson-Romberg extrapolation acts orthogonally, providing a second-order reduction in its bias. In this work, we show that their composition is strictly better than both, not only maintaining the enhanced MSE guarantees but also yielding an even greater cubic refinement in the bias. To the best of our knowledge, our work provides the first theoretical guarantees for such a synergy in structured non-monotone VIPs. Our analysis proceeds in two steps: (i) we smooth the discrete noise induced by reshuffling and leverage tools from continuous-state Markov chain theory to establish a novel law of large numbers and a central limit theorem for its iterates; and (ii) we employ spectral tensor techniques to prove that extrapolation debiases and sharpens the asymptotic behavior even under the biased gradient oracle induced by reshuffling. Finally, extensive experiments validate our theory, consistently demonstrating substantial speedups in practice.

==> Shuffle_the_Data_arxiv_version_/acknowledgments.tex <==
\subsubsection*{Acknowledgments}
Konstantinos Emmanouilidis and Ren\'{e} Vidal acknowledge support from the NSF-Simons grant 2031985 ``Research Collaborations on the Mathematical and Scientific Foundations of Deep Learning" and Simons Foundation 81420 (Theorinet). Emmanouil-Vasileios Vlatakis-Gkaragkounis acknowledges support from the startup funding at Wisconsin Madison university under the grant (233-AAN5596 - GF000020971).
\newpage

==> Shuffle_the_Data_arxiv_version_/algo_figure.tex <==
% !TEX root = ./iclr2026_conference.tex

\usetikzlibrary{calc,backgrounds,decorations.pathreplacing,positioning}
\begin{tikzpicture}[
  >={stealth}, font=\small,
  box/.style={draw, rounded corners=5pt, align=center, inner sep=7pt, minimum height=1.15cm},
  epoch/.style={box, text width=2.55cm, fill=blue!8, draw=blue!40!black, thick},
  epochB/.style={box, text width=2.55cm, fill=orange!9, draw=orange!70!black, thick},
  extbox/.style={box, text width=4.0cm, fill=green!9, draw=green!45!black, thick},
  outbox/.style={box, text width=2.1cm, fill=gray!9, draw=gray!50, thick},
  permbox/.style={box, text width=2.3cm, fill=violet!8, draw=violet!50!black, thick},
]
\colorlet{cA}{blue!65!black}
\colorlet{cB}{orange!75!black}
\colorlet{cE}{green!45!black}
\colorlet{cG}{gray!55!black}
\colorlet{cP}{violet!70!black}

% ── Global shift: centre the diagram (content spans ~0..15.5, shift left 1.7cm)
\begin{scope}[xshift=-1.7cm]

%% ---- header A
\node[cA, font=\small\bfseries] (hA) at (4.1, 0.62)
  {SGD-\texttt{RR\textsubscript{1}} inner loop \enspace (step $\gamma$)};

%% ---- Run A epochs
\node[epoch] (A1) at (0,   -0.5) {Epoch $k{-}1$\\[2pt]{\footnotesize $n$ steps, step $\gamma$}};
\node[epoch] (A2) at (3.85,-0.5) {Epoch $k$\\[2pt]{\footnotesize $n$ steps, step $\gamma$}};
\node[epoch] (A3) at (7.70,-0.5) {Epoch $k{+}1$\\[2pt]{\footnotesize $n$ steps, step $\gamma$}};

\draw[cA, very thick, ->] (A1.east) -- (A2.west)
  node[midway, above=3pt, font=\scriptsize, cA] {$x_k^{[\gamma]}$};
\draw[cA, very thick, ->] (A2.east) -- (A3.west)
  node[midway, above=3pt, font=\scriptsize, cA] {$x_{k+1}^{[\gamma]}$};

%% ---- inner step equation box
\node[draw=cA!60, fill=blue!1, rounded corners=3pt,
      font=\scriptsize, inner sep=5pt, align=center, text width=3.2cm]
  (inner) at (5.5,-2.8)
  {$x_k^{i+1}\!\gets\!x_k^i- \eta F_{\omega_k[i]}(x_k^i)$\\ \vspace{.05cm} \hspace{.5pt} $i=0,\dots,n{-}1$};
%\draw[cA!50, dashed, ->] (A2.south) to[out=270,in=110] (inner.north west);

%% ---- Shared ω_k box: LEFT of inner equation, violet
\node[permbox] (perm) at (1.8,-2.8)
  {\textbf{Shared} $\omega_k$\\[3pt]across both runs};

% → equation
\draw[cP, thick, ->] (perm.east) -- (inner.west);
% ↑ Run A
\draw[cP, thick, ->] (perm.north) to[out=90,in=200] (A2.south west);

%% ---- orange header: well above orange boxes
\node[cB, font=\small\bfseries] (hB) at (4.1,-6.30)
  {SGD-\texttt{RR\textsubscript{1}} inner loop \enspace (step $2\gamma$)};

%% ---- Run B epochs
\node[epochB] (B1) at (0,   -5.40) {Epoch $k{-}1$\\[2pt]{\footnotesize $n$ steps, step $2\gamma$}};
\node[epochB] (B2) at (3.85,-5.40) {Epoch $k$\\[2pt]{\footnotesize $n$ steps, step $2\gamma$}};
\node[epochB] (B3) at (7.70,-5.40) {Epoch $k{+}1$\\[2pt]{\footnotesize $n$ steps, step $2\gamma$}};

% ↓ Run B
\draw[cP, thick, ->] (perm.south) to[out=270,in=145] (B2.north west);

\draw[cB, very thick, ->] (B1.east) -- (B2.west)
  node[midway, below=3pt, font=\scriptsize, cB] {$x_k^{[2\gamma]}$};
\draw[cB, very thick, ->] (B2.east) -- (B3.west)
  node[midway, below=3pt, font=\scriptsize, cB] {$x_{k+1}^{[2\gamma]}$};

%% ---- Extrapolation block (vertically centred between A3 and B3)
\node[extbox, minimum height=3.2cm, text width=4.0cm] (ext) at (13.1,-2.95)
  {\textbf{RR\textsubscript{2} Extrapolation}\\[8pt]
   $\hat{x}_{k+2} = 2\,x_{k+2}^{[\gamma]} - x_{k+2}^{[2\gamma]}$\\[8pt]
   {\small Cancels $\mathcal{O}(\gamma)$ bias term}\\[4pt]
   {\small Bias: $\mathcal{O}(\gamma)\to\mathcal{O}(\gamma^3)$}};

\draw[cA, very thick, ->] (A3.east) to[out=0,in=145]
  node[above=4pt,font=\scriptsize,cA] {$x_{k+2}^{[\gamma]}$} (ext.north west);
\draw[cB, very thick, ->] (B3.east) to[out=0,in=215]
  node[below=4pt,font=\scriptsize,cB] {$x_{k+2}^{[2\gamma]}$} (ext.south west);

%% ---- output
\node[outbox] (out) at (13.1,1.15)
  {\textbf{Output} $\hat{x}_K$\\[3pt]{\small Bias $\mathcal{O}(\gamma^3)$}};
\draw[cE, very thick, ->] (ext.north) -- (out.south)
  node[midway, right=4pt, font=\scriptsize, cE] {\textbf{return}};

%% ---- comparison table (centred under the main diagram)
\node[draw=cG, fill=gray!4, rounded corners=5pt, inner sep=7pt,
      font=\footnotesize, align=center] at (6,2.4)
  {\begin{tabular}{lcccc}
     \textbf{Method} &
     \textbf{SGD} &
     \textbf{SGD-\texttt{RR\textsubscript{1}}} &
     \textbf{SGD-\texttt{RR\textsubscript{2}}} &
     \textbf{SGD-\texttt{RR\textsubscript{2}$\oplus$RR\textsubscript{1}}} \\[4pt]
     \hline\\[-5pt]
     Bias  & $\mathcal{O}(\gamma)$ & $\mathcal{O}(\gamma)$ & $\mathcal{O}(\gamma^{3/2})$ &$\boldsymbol{\mathcal{O}(\gamma^3)}$ \\[2pt]
     MSE   & $\mathcal{O}(\gamma)$ & $\mathcal{O}(\gamma^2)$ & $\mathcal{O}(\gamma)$ & $\boldsymbol{\mathcal{O}(\gamma^2)}$
   \end{tabular}};

\end{scope}
\end{tikzpicture}


==> Shuffle_the_Data_arxiv_version_/conclusion.tex <==
% !TEX root = ./iclr2026_conference.tex
% \vspace{-1em}
\section{Conclusion}
% \vspace{-0.75em}
In summary, our work establishes that the synergy of random reshuffling and extrapolation yields a principled reduction of bias, culminating in accelerated convergence guarantees for structured non-monotone VIPs.  
By combining Markov chain techniques, spectral analysis, and higher-moment bounds, we provide the first rigorous evidence that these heuristics can be synergistically integrated rather than studied in isolation.  
This perspective bridges a long-standing gap between practice and theory, offering a systematic framework that extends naturally to a broad class of constant step-size stochastic methods.  
We view this as a foundation for a new generation of analyses where practical heuristics are not only empirically verified but also theoretically grounded to deliver provable performance improvements in complex stochastic optimization landscapes.

==> Shuffle_the_Data_arxiv_version_/experiments.tex <==
% !TEX root = ./iclr2026_conference.tex


\section{Experiments}
\begin{figure}[b!]
    \centering
    \includegraphics[width=0.3\linewidth]{./figures/relative_error_plots/new_plot_manolis_gamma_0.0013714594258871589_condition_num_1.pdf.pdf}
    \includegraphics[width=0.3\linewidth]{./figures/relative_error_plots/new_plot_manolis_gamma_0.00037627352424815026_condition_num_5.pdf.pdf}
    \includegraphics[width=0.3\linewidth]{./figures/relative_error_plots/new_plot_manolis_gamma_0.0001_condition_num_10.pdf.pdf}
    \caption{Comparison of different heuristics. The combination of \RRrom$\oplus$\RRresh\ converges linearly to neighborhood of the solution, validating the established theoretical results (Theorem~\ref{thm: convergence_rate}). Even when we are using the last iterates, the combination of \RRrom$\oplus$\RRresh\ converges to a smaller relative error in comparison to the other variants (classical SGDA, \RRresh, \RRrom). This validates that the bias of Algorithm~\ref{alg:rrrom-rrresh} is improved even when \RRresh-last iterates are used. }
    \label{fig: rate_of_conv}
\end{figure}
In this section, we conduct a series of experiments demonstrating the benefits from the synergy of the two heuristics empirically. 
More specifically, we focus in the strongly monotone setting and compare the relative error and bias attained by 4 variants: the classical SGD(A) algorithm using uniform with-replacement sampling (denoted as \emph{SGDA} in the plots), the one equipped with \RRresh, the one equipped with \RRrom\ and the method utilizing both heuristics. 
For each experiment, we report the average of $5$ trials/runs and plot the relative error $\log\left(\frac{\|x_k - x^*\|^2}{\|x_0 - x^*\|^2}\right)$ with respect to the iterations of the algorithm.

\textbf{\textit{Two-player Zero-Sum Games.}} In the strongly monotone case, we consider the two-player zero-sum game from \cite{emmanouilidis2024stochastic} and \cite{loizou2021stochastic}, consisting a strongly convex - strongly concave quadratic of the form
\begin{eqnarray}
    \min_{x_{1} \in \R^d} \max_{x_{2}\in \R^d} f(x_1, x_2) = \frac{1}{n} \sum_{i=1}^{n} \frac{1}{2} x_1^T A_i x_1 + x_1^T B_i x_2 - \frac{1}{2} x_2^T C_i x^2 + \alpha_i^T x_1 - c_i^T x_2. \nonumber
\end{eqnarray}
For the interested reader, additional details on the experimental setup and the procedure used to sample the matrices $A_i, B_i, C_i$ are provided in Appendix~\ref{app: additional_experiments}.

\textbf{On the Rate of Convergence.} In the first set of experiments, we aim to validate empirically the result of Theorem~\ref{thm: convergence_rate} by running SGDA with \RRresh\ and using the step sizes described by theory. We conduct experiments for multiple conditions $\kappa = \frac{L}{\mu}$ with value $\kappa = \{1, 5, 10\}$ and $\mu = 1$. In Figure~\ref{fig: rate_of_conv}, we observe that the algorithm with \RRresh\ converges linearly to a neighbourhood around the solution $x^*$ and the neighbourhood depends on the step size used, validating in this way the results of Theorem~\ref{thm: convergence_rate}. We have run experiments also for stepsizes that are larger than the ones predicted in theory, observing similar behaviour of the optimization algorithm. Additionally, we have performed an ablation study in Wasserstein GANs \citep{emmanouilidis2024stochastic, daskalakis2017training}, showing that the performance benefit of the proposed heuristic is universal in many other common optimization algorithms used in VIs (Appendix~\ref{app: additional_experiments}).


\textbf{Efficient Statistics \& Empirical Concentration.} This set of experiments examines the central limit theorem (CLT) and aims to validate empirically the theoretical results established in Theorem~\ref{thm: LLN_CLT_res}. The value of the game, which is zero, is used as the test value for which we observe the averaged evaluations after $T = \{100, 500, 1000\}$ iterations respectively. In particular, we run the algorithm with the step size suggested by Theorem~\ref{thm: LLN_CLT_res} and maintain for the total number of iterations the sum of the evaluations, normalized with $\sqrt{T}$. We run the experiment for $T = 2000$ trials/runs and plot the corresponding histograms. In Figure~\ref{fig: clt_validation}, we observe that the histograms tend to concentrate to the value of the game as the number of iterations increase. Additionally, we examine the effect of the step size to concentration of the observed distributions. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.35\linewidth]{./figures/concentration/fig3_sgda_4.pdf}
    \includegraphics[width=0.3\linewidth]{./figures/concentration/fig4_sgda_4.pdf}
    \caption{Validation of concentration around the mean and effect of the number of iterations and step sized selected. The average of the game values tend to concentrate more around the mean for larger number of iterations and smaller step sizes. The right plot indicates the effect of two different step sizes $\gamma \in \{0.1, 0.001\}$, showing that for smaller step sizes the corresponding distribution attains higher concentration around the mean of the values.}
    \label{fig: clt_validation}
\end{figure}


==> Shuffle_the_Data_arxiv_version_/gamma-neighbors.tex <==
% !TEX root = ./iclr2026_conference.tex

\tikzset{every picture/.style={line width=0.75pt}}        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]


%Shape: Ellipse [id:dp7329906304802944] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.29 ] (481.22,393.5) .. controls (481.22,299.89) and (557.06,224) .. (650.61,224) .. controls (744.16,224) and (820,299.89) .. (820,393.5) .. controls (820,487.11) and (744.16,563) .. (650.61,563) .. controls (557.06,563) and (481.22,487.11) .. (481.22,393.5) -- cycle ;
%Shape: Ellipse [id:dp14673386188875415] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.41 ] (537.7,393.5) .. controls (537.7,331.1) and (588.25,280.52) .. (650.61,280.52) .. controls (712.97,280.52) and (763.52,331.1) .. (763.52,393.5) .. controls (763.52,455.9) and (712.97,506.48) .. (650.61,506.48) .. controls (588.25,506.48) and (537.7,455.9) .. (537.7,393.5) -- cycle ;
%Shape: Ellipse [id:dp3138874134344609] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (568.79,393.5) .. controls (568.79,348.28) and (605.42,311.62) .. (650.61,311.62) .. controls (695.8,311.62) and (732.44,348.28) .. (732.44,393.5) .. controls (732.44,438.72) and (695.8,475.38) .. (650.61,475.38) .. controls (605.42,475.38) and (568.79,438.72) .. (568.79,393.5) -- cycle ;
%Shape: Ellipse [id:dp6951380714624634] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.73 ] (617.47,393.5) .. controls (617.47,375.18) and (632.31,360.34) .. (650.61,360.34) .. controls (668.91,360.34) and (683.75,375.18) .. (683.75,393.5) .. controls (683.75,411.82) and (668.91,426.66) .. (650.61,426.66) .. controls (632.31,426.66) and (617.47,411.82) .. (617.47,393.5) -- cycle ;

% =============== COLORED POLYLINES WITH STARS ===============

% Green path
\draw [color={rgb, 255:red, 110; green, 192; blue, 19 }, line width=2.25]
  (356,490) -- (341,370) -- (418,243) -- (508,191) -- (594,212) -- (626.22,296.33);
\foreach \p in {(356,490),(341,370),(418,243),(508,191),(594,212),(626.22,296.33)}{
  \node[star, star points=5, draw={rgb,255:red,110; green,192; blue,19},
        fill={rgb,255:red,110; green,192; blue,19}, minimum size=7pt, inner sep=0pt] at \p {};
}

% Blue path
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }, line width=2.25]
  (356,490) -- (321,336) -- (362,258) -- (424,199) -- (499,157) -- (607,151)
  -- (698,178) -- (728,218) -- (713.68,258.29);
\foreach \p in {  (356,490) , (321,336) , (362,258) , (424,199) , (499,157) , (607,151)
  , (698,178) , (728,218) , (713.68,258.29)}{
  \node[star, star points=5, draw={rgb,255:red,74; green,144; blue,226},
        fill={rgb,255:red,74; green,144; blue,226}, minimum size=7pt, inner sep=0pt] at \p {};
}

% Orange path
\draw [color={rgb, 255:red, 206; green, 131; blue, 13 }, line width=2.25]
  (356,490) -- (388,387) -- (498,266) -- (574,267) -- (601,279) -- (618.6,339.2);
\foreach \p in {(356,490),(388,387),(498,266),(574,267),(601,279),(618.6,339.2)}{
  \node[star, star points=5, draw={rgb,255:red,206; green,131; blue,13},
        fill={rgb,255:red,206; green,131; blue,13}, minimum size=7pt, inner sep=0pt] at \p {};
}

% Red path
\draw [color={rgb, 255:red, 165; green, 6; blue, 24 }, line width=2.25]
  (356,490) -- (420,388) -- (504,346) -- (580,343) -- (641.61,376.61);
\foreach \p in {(356,490),(420,388),(504,346),(580,343),(641.61,376.61)}{
  \node[star, star points=5, draw={rgb,255:red,165; green,6; blue,24},
        fill={rgb,255:red,165; green,6; blue,24}, minimum size=7pt, inner sep=0pt] at \p {};
}

% =============================================================
%
%% Text Node
%\draw (632.38,393.8) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ]  {$x_{*}$};
%% Text Node
%\draw (606.03,200.22) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,rotate=-0.45]  {$\mathrm{bias}( \gamma ) =\ \mathcal{O}\left( \gamma \right)$};
%% Text Node
%\draw (671.93,254.71) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 100; green, 172; blue, 43 },opacity=1 ,rotate=-25.81]  {$\mathrm{bias}( \gamma ) =\ \mathcal{O}\left( \gamma ^{1.5}\right)$};
%% Text Node
%\draw (598.56,429.08) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ,rotate=-0.61]  {$\mathrm{bias}( \gamma ) =\ \mathcal{O}\left( \gamma ^{3}\right)$};
%% Text Node
%\draw (720.43,309.21) node [anchor=north west][inner sep=0.75pt]  [font=\large,color={rgb, 255:red, 231; green, 151; blue, 19 }  ,opacity=1 ,rotate=-60.58]  {$\mathrm{bias}( \gamma ) =\ \mathcal{O}\left( \gamma ^{2}\right)$};
%% Text Node
%\draw (372.38,478.8) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$x_{0}$};

% Text Node
\draw (632.38,393.8) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ]  {$x_{*}$};
% Text Node
\draw (606.03,200.22) node [anchor=north west][inner sep=0.75pt]  [font=\large,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,rotate=-0.45]  {$\mathrm{bias}( \gamma ) =\ O( \gamma )$};
% Text Node
\draw (665.93,244.71) node [anchor=north west][inner sep=0.75pt]  [font=\large,color={rgb, 255:red, 83; green, 146; blue, 2 }  ,opacity=1 ,rotate=-25.81]  {$\mathrm{bias}( \gamma ) =\ O\left( \gamma ^{1.5}\right)$};
% Text Node
\draw (595.56,429.08) node [anchor=north west][inner sep=0.75pt]  [font=\large,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ,rotate=-0.61]  {$\mathrm{bias}( \gamma ) =\ O\left( \gamma ^{3}\right)$};
% Text Node
\draw (716.43,301.21) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 180; green, 117; blue, 0 }  ,opacity=1 ,rotate=-60.58]  {$\mathrm{bias}( \gamma ) =\ O\left( \gamma ^{2}\right)$};
% Text Node
\draw (365.38,478.8) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$x_{0}$};

%Straight Lines [id:da7873343135782715] 
\draw    (650.61,393.5) -- (648.05,234) ;
\draw [shift={(648,231)}, rotate = 89.08] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
\draw [shift={(650.61,393.5)}, rotate = 269.08] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da8747548930371518] 
\draw    (650.61,393.5) -- (695.72,297.71) ;
\draw [shift={(697,295)}, rotate = 115.22] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
\draw [shift={(650.61,393.5)}, rotate = 295.22] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da18150789044644122] 
\draw    (650.61,393.5) -- (713.61,347.16) ;
\draw [shift={(716.03,345.38)}, rotate = 143.66] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
\draw [shift={(650.61,393.5)}, rotate = 323.66] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da6863210759512379] 
\draw    (650.61,393.5) -- (665.12,418.22) ;
\draw [shift={(666.64,420.81)}, rotate = 239.59] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
\draw [shift={(650.61,393.5)}, rotate = 59.59] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;



% % Central point and labels
% \draw (632.38,393.8) node [anchor=north west][inner sep=0.75pt] [font=\large,color=white] {$x_{*}$};
% \draw (606.03,200.22) node [anchor=north west][font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }] {$\mathrm{bias}( \gamma ) =\ O( \gamma )$};
% \draw (671.93,254.71) node [anchor=north west][font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }] {$\mathrm{bias}( \gamma ) =\ O\!\left( \gamma ^{1.5}\right)$};
% \draw (598.56,429.08) node [anchor=north west][font=\footnotesize,color={rgb, 255:red, 208; green, 2; blue, 27 }] {$\mathrm{bias}( \gamma ) =\ O\!\left( \gamma ^{3}\right)$};
% \draw (720.43,309.21) node [anchor=north west][font=\footnotesize,color={rgb, 255:red, 231; green, 151; blue, 19 }] {$\mathrm{bias}( \gamma ) =\ O\!\left( \gamma ^{2}\right)$};
% \draw (372.38,478.8) node [anchor=north west][font=\large,color=black] {$x_{0}$};

\end{tikzpicture}

==> Shuffle_the_Data_arxiv_version_/introduction.tex <==
% !TEX root = ./iclr2026_conference.tex


\section{Introduction}
Variational inequality problems (VIPs) \citep{stampacchia1964formes} are a 
% Mathematical optimization is one of the pillars of modern machine learning (ML), equipping us with the numerical tools needed to compute parameters for large-scale decision systems. In this work, we focus on \emph{variational inequality problems (VIPs)} \citep{stampacchia1964formes}—
unifying framework that extends beyond classical loss minimization to encompass min–max optimization, complementarity problems \citep{dantzig1968complementary,facchinei2003finite}, equilibrium computation in games, and general fixed-point formulations  \citep{bauschke2017convex}. In recent years, VIPs have gained significant traction in ML and data science, especially due to their broad potential applicability in domains where minimizing a single empirical loss is insufficient. Notable examples
% , with notable examples including 
include generative adversarial networks \citep{goodfellow2014generative,arjovsky2017wasserstein}, multi-agent and robust reinforcement learning \citep{namkoong2016stochastic,wang2021adversarial,giannou2022convergence}, and auction theory \citep{syrgkanis2015fast}.

In practice, many of these tasks reduce to finite-sum formulations, where the objective depends on a large collection of data samples or agents. In such settings, \emph{stochastic gradient methods} have become the workhorse of large-scale learning \citep{bottou2018optimization}. By exploiting the finite-sum structure, stochastic gradient descent (SGD) and its variants replace expensive full-gradient computations with inexpensive updates on a few components, enabling scalability to massive datasets. 

\kostas{While the theoretical underpinnings of SGD date back to the seminal work of \citet{robbins1951stochastic} and \citet{kiefer1952stochastic}, the initial results involved an asymptotic analysis under a vanishing step size. Consequent works \citep{ljung1978strong, benaim2006dynamics, rakhlin2011making,raginsky2017non,azizian2024long,MalickMertikopoulos2024} have extended the guarantees of SGD under different design choices,} since much of its practical success can be traced to a handful of seemingly “low-level” heuristics \citep{bottou2012stochastic}: step-size schedules (constant vs.\ decaying), data ordering (with vs.\ without resampling), and iterate selection (average vs.\ last iterate). To facilitate analysis, the community has typically adopted a \emph{ceteris paribus} perspective—isolating one design choice at a time while holding the rest fixed—an approach that clarifies individual effects but obscures their interaction.

A particularly important case is the use of a \emph{constant step size} $\gamma$, which is popular in practice since it simplifies tuning, quickly erases the dependence on initialization, and yields fast early progress \citep{yu2021analysis}. However, its fundamental drawback is that convergence halts at a non-vanishing error. Even in strongly convex problems with unique solution $x^*$, the last iterate of SGD typically satisfies: \[\text{$\text{MSE}(\texttt{SGD})=\limsup_{k\to\infty}\ex[\|x_k-x^*\|^2]=\mathcal{O}(\gamma)$ and $\text{bias}(\texttt{SGD})=\limsup_{k\to\infty}\|\ex[x_k]-x^*\|=\mathcal{O}(\gamma)$.}\] That is, the iterates stabilize at a distance from the optimum on the order of the step size.


$\blacktriangleright$ To mitigate this limitation, practitioners often turn to debiasing heuristics.  A prominent example is \emph{random reshuffling} (\RRresh), or \emph{without-replacement} sampling, where each data point is visited exactly once per epoch. Unlike classical \emph{with-replacement} SGD, which may resample or skip points, \RRresh\ enforces a random full pass that closely mirrors large-scale training in practice \citep{bottou2018optimization}. Despite the dependence it induces across samples, recent work has established faster convergence guarantees for \RRresh\ in both minimization \citep{ahn2020sgd,gurbuzbalaban2021random,cai2023empirical} and VIPs \citep{mishchenko2020revisiting,emmanouilidis2024stochastic}, along with sharper \emph{MSE} bounds from $\mathcal{O}(\gamma)$ to $\mathcal{O}(\gamma^2)$.
However, the question of whether the bias term improves has remained open.
%, while leaving open the question of whether the bias term itself improves. 
Indeed, recall that for any estimator $\hat x$, the mean squared error decomposes as
\[
\mathrm{MSE}(\hat x) \;=\; \ex[\|\hat x - x^*\|^2] \;=\; \|\ex[\hat x]-x^*\|^2 \;+\; \mathrm{Var}(\hat x),
\]
so that $\mathrm{bias}(\hat x) \le \sqrt{\mathrm{MSE}(\hat x)}$. Under this trivial bound, \textsc{SGD–\RRresh} guarantees improved MSE compared to vanilla SGD, but does not necessarily yield smaller bias.


$\blacktriangleright$ Orthogonal to reshuffling, another classical idea from numerical analysis has recently re-emerged in stochastic optimization: \emph{\citeauthor{richardson1911ix}–\citeauthor{romberg1955vereinfachte}} (\RRrom) \emph{extrapolation}. Its principle is simple yet powerful: \emph{Run the algorithm of your choice with two different step sizes and combine their outputs so that the leading bias term cancels.} Concretely, whenever the bias admits an expansion of the form $\text{bias}(\gamma) = \Delta \gamma + \mathcal{O}(\gamma^{\kappa})$ with $\kappa>1$, running the stochastic approximation at two step sizes gives:
\[\text{$x_{\infty}^{\gamma} - x^* = \Delta \gamma + \mathcal{O}(\gamma^{\kappa})$ and $x_{\infty}^{2\gamma} - x^* = 2\Delta \gamma + \mathcal{O}(\gamma^{\kappa})$.}\vspace{-0.25em}\] 
Extrapolating these iterates then yields: 
\[
x_{\text{extr}}- x^*
= 2x_{\infty}^{\gamma} - x_{\infty}^{2\gamma} - x^*
= \cancel{2\Delta \gamma} - \cancel{2\Delta \gamma} + \mathcal{O}(\gamma^{\kappa})
= \mathcal{O}(\gamma^{\kappa}).
\]
Originally introduced for accelerating discretization schemes in stochastic differential equations \citep{hildebrand1987introduction,talay1990expansion,bally1996law}, \RRrom\ has since been applied to optimization, improving constant-step methods from SGD \citep{durmus2016stochastic,dieuleveut2020bridging,mangold2024refined,sheshukova2024nonasymptotic} to Q-learning and two-timescale stochastic approximation methods \citep{huo2023bias,kwon2024two,zhang2024constant,allmeier2024computing}. 
However, despite its conceptual simplicity and empirical success, the theoretical foundations of \RRrom\ for stochastic VIPs remain nascent \citep{vlatakis2024stochastic}. 

In summary, the known \emph{bias} rates of the heuristics remain limited when they are applied in isolation:
For unconstrained strongly monotone VIPs, \RRresh\ is known to sharpen \emph{MSE} bounds (from $\mathcal{O}(\gamma)$ to $\mathcal{O}(\gamma^2)$) but does not, in general, guarantee an improved bias order; on the other hand \RRrom\ alone attains $\mathcal{O}(\gamma^{3/2})$ bias \citep{vlatakis2024stochastic}\footnote{The $\mathcal{O}(\gamma^2)$ rate in \citet[Sec.~5, Thm.~6]{vlatakis2024stochastic} is obtained via a reduction to \citet[Sec.~3, Thm.~4]{dieuleveut2020bridging}, which requires additional noise assumptions not met in our setting.}.
\kostas{However, it remains unclear whether one can combine effectively the aforementioned heuristics in a unified method that outperforms both, ideally reaching $\mathcal{O}(\gamma^{3})$ bias. This raises the natural question:} 
$$$$
\begin{equation}
\parbox{35em}{\centering
\textit{What new phenomena arise when these heuristics\\—
\emph{constant step sizes, random reshuffling, and Richardson extrapolation}—\\
interact simultaneously?}
}
\tag{$\bigstar$}
\label{central-question}
\end{equation}
\\\\
Addressing this question is delicate, because reshuffling introduces a biased stochastic oracle whose discrete, permutation-driven noise structure is not covered by
existing analyses of extrapolation, which predominantly assume unbiased or continuously distributed perturbations \citep{dieuleveut2020bridging,sheshukova2024nonasymptotic,vlatakis2024stochastic}.
\newpage

\textbf{Our contributions.}
In this work, we unify the \RRresh\ and \RRrom\ heuristics into a principled algorithmic framework, showing that their composition yields a level of bias reduction unattainable by either heuristic alone.

\begin{maininformal}
Let $F$ be a quasi-strongly monotone smooth finite-sum operator.
Run \textup{SGD-}\RRrom$\oplus$\RRresh\ \textup{(Algorithm~\ref{alg:rrrom-rrresh})} with
two parallel step sizes $\gamma$ and $2\gamma$, and combine their epoch-level
outputs via Richardson–Romberg extrapolation. Then $\exists\; c,c'<\infty$,
$\rho,\rho'\in(0,1)$ such that:
\[
  \underbrace{\bigl\|\mathbb{E}[x_k]-x^*\bigr\|}_{\displaystyle\mathrm{bias}}
  \;\leq\; c\,(1-\rho)^k \;+\; \mathcal{O}(\gamma^3),
  \qquad
  \underbrace{\mathbb{E}\bigl[\|x_k-x^*\|^2\bigr]}_{\displaystyle\mathrm{MSE}}
  \;\leq\; c'(1-\rho')^k \;+\; \mathcal{O}(\gamma^2).
\]
The $\mathcal{O}(\gamma)$ and $\mathcal{O}(\gamma^2)$ bias terms cancel exactly via extrapolation,
yielding a strictly cubic improvement over \RRresh\ alone $(\mathcal{O}(\gamma))$
and \RRrom\ alone $(\mathcal{O}(\gamma^{3/2}))$, while preserving the $\mathcal{O}(\gamma^2)$ MSE of \RRresh.
\end{maininformal}


\medskip
\noindent\textbf{Our contributions are as follows:}

\noindent$\star$ \emph{Convergence of SGD-\RRresh\ under perturbations.}
We analyze the \RRresh\ component, proving exponential convergence with an $\mathcal{O}(\gamma^2)$ bias under quasi-strong monotonicity, robust to preprocessing perturbations.

\noindent$\star$ \emph{Epoch-level Markov chain analysis of SGD-\RRresh.}
We prove that the dynamics of \RRresh\ admit a unique invariant stationary distribution and establish a Law of Large Numbers (LLN) and a Central Limit Theorem (CLT) for the per-epoch iterates.

\noindent$\star$ \emph{Cubic bias refinement via \RRrom$\oplus$\RRresh\ synergy.}
Through a spectral analysis of the reshuffling-induced biased oracle and higher-moment bounds, we prove the first $\mathcal{O}(\gamma^3)$ asymptotic bias guarantee for the combined algorithm in quasi-strongly monotone VIPs.

==> Shuffle_the_Data_arxiv_version_/limitations.tex <==
\section*{Limitations}
\paragraph{Limitations of the structural assumption.}
A central structural assumption in our analysis is that the operator $F$ satisfies 
$\lambda$-weak $\mu$-quasi-strong monotonicity. This condition is broad enough to include 
several meaningful non-monotone problem classes—such as dissipative dynamical systems, 
weakly convex optimization, and locally contractive variational inequalities—and is standard 
in modern analyses of stochastic fixed-point and operator-splitting methods 
(e.g., Hsieh et al., 2019; Mertikopoulos and Zhou, 2019; Chavdarova et al., 2021). 
However, it is important to emphasize the following limitations.

\begin{enumerate}
    \item \textbf{Not applicable to general nonconvex--nonconcave min--max problems.}  
    The assumption does \emph{not} hold for arbitrary adversarial problems such as deep GANs, 
    multi-agent RL environments, or smooth non-monotone games with persistent rotational dynamics. 
    These settings may lack even local stability 
    (e.g., Daskalakis et al.\ 2018; Fiez et al.\ 2020). 
    Accordingly, our theoretical guarantees should not be interpreted as applying to fully adversarial 
    or worst-case min--max formulations.

    \item \textbf{Local nature of the assumption.}  
    Quasi-strong monotonicity is inherently a \emph{local} regularity condition: smooth operators 
    that are monotone in a neighborhood of a solution satisfy it on that region 
    (Lemma~A.4, Hsieh et al.\ 2019). This requires smoothness and regularity that may not hold in 
    problems involving discontinuities, clipping, piecewise-linear losses, or hard constraints. 
    In such cases, the assumption may fail even locally.

    \item \textbf{Not capturing highly oscillatory or anti-monotone operators.}  
    Allowing $\lambda>0$ permits controlled violation of monotonicity, but the assumption still 
    does not model strongly anti-monotone or highly oscillatory operators. Extending our analysis to 
    Minty variational inequalities, hypomonotone operators, or other generalized monotonicity 
    classes remains an interesting direction for future work.
\end{enumerate}

Despite these limitations, we believe the assumption remains meaningful for a broad set of 
structured, smooth VIPs where local stability is present. We hope that this explicit discussion 
helps avoid any misunderstanding about the scope of applicability of our results.


==> Shuffle_the_Data_arxiv_version_/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Shuffle_the_Data_arxiv_version_/model.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,711); %set diagram left start at 0, and has height of 711

%Shape: Rectangle [id:dp7167201570186642] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.24 ] (24,362) -- (832,362) -- (832,548) -- (24,548) -- cycle ;
%Straight Lines [id:da5348252051360501] 
\draw    (215.16,530) -- (642,530) ;
%Straight Lines [id:da5870165356755055] 
\draw    (642,530) -- (783.02,530) ;
\draw [shift={(717.51,530)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Shape: Rectangle [id:dp22967037843062987] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.71 ] (90.45,408.54) -- (296.62,408.54) -- (296.62,493.84) -- (90.45,493.84) -- cycle ;
%Straight Lines [id:da17785199775015115] 
\draw    (74.14,477.2) -- (133.09,477.2) ;
\draw [shift={(136.09,477.2)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Shape: Rectangle [id:dp2742561061453428] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.3 ] (136.49,440.15) -- (233.94,440.15) -- (233.94,486.86) -- (136.49,486.86) -- cycle ;

%Straight Lines [id:da09921992906541832] 
\draw    (102.26,465.12) -- (133.9,465.12) ;
\draw [shift={(136.9,465.12)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da337709340044827] 
\draw    (234.35,465.12) -- (260.64,465.12) ;
\draw [shift={(263.64,465.12)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da8354383452527102] 
\draw    (240.28,465.12) -- (281.06,465.12) ;
%Straight Lines [id:da8152793732524597] 
\draw    (281.06,465.12) -- (281.06,425.65) ;
%Straight Lines [id:da7570544004782095] 
\draw    (102.26,465.12) -- (102.26,424.85) ;
%Straight Lines [id:da4721478714710243] 
\draw    (281.06,425.65) -- (102.26,425.65) ;
%Straight Lines [id:da3188806653380546] 
\draw    (281.06,465.12) -- (328.05,465.12) ;
\draw [shift={(331.05,465.12)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da5695989834818472] 
\draw    (52.27,465.12) -- (102.26,465.12) ;
%Straight Lines [id:da005449392824766197] 
\draw    (52.27,465.12) -- (52.27,398.2) ;
%Straight Lines [id:da5087383745711406] 
\draw    (331.05,465.12) -- (331.05,398.2) ;
%Straight Lines [id:da7805722702952284] 
\draw    (331.05,398.2) -- (52.27,398.2) ;
%Straight Lines [id:da42790020085683145] 
\draw    (52.27,465.12) -- (24.08,465.12) ;
%Shape: Rectangle [id:dp8867101993788168] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.71 ] (766.71,408.41) -- (560.54,408.41) -- (560.54,493.71) -- (766.71,493.71) -- cycle ;
%Straight Lines [id:da45046936384949954] 
\draw    (783.02,477.06) -- (724.07,477.06) ;
\draw [shift={(721.07,477.06)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Shape: Rectangle [id:dp8984113920591881] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.3 ] (623.21,440.01) -- (720.67,440.01) -- (720.67,486.73) -- (623.21,486.73) -- cycle ;

%Straight Lines [id:da49889800256014705] 
\draw    (754.89,464.98) -- (723.26,464.98) ;
\draw [shift={(720.26,464.98)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da31365561028594713] 
\draw    (622.81,464.98) -- (596.52,464.98) ;
\draw [shift={(593.52,464.98)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da9666480403965403] 
\draw    (616.88,464.98) -- (576.1,464.98) ;
%Straight Lines [id:da6870758288531431] 
\draw    (576.1,464.98) -- (576.1,425.52) ;
%Straight Lines [id:da13859487218454614] 
\draw    (754.89,464.98) -- (754.89,424.71) ;
%Straight Lines [id:da30734305051591637] 
\draw    (576.1,425.52) -- (754.89,425.52) ;
%Straight Lines [id:da11442520008239165] 
\draw    (576.1,464.98) -- (529.1,464.98) ;
\draw [shift={(526.1,464.98)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da11238862430956253] 
\draw    (804.89,464.98) -- (754.89,464.98) ;
%Straight Lines [id:da3927723255927097] 
\draw    (804.89,464.98) -- (804.89,398.06) ;
%Straight Lines [id:da17493801390941033] 
\draw    (526.1,464.98) -- (526.1,398.06) ;
%Straight Lines [id:da38944767089549004] 
\draw    (526.1,398.06) -- (804.89,398.06) ;
%Straight Lines [id:da5789729604768556] 
\draw    (298.12,465.45) -- (526.1,464.98) ;
%Straight Lines [id:da5056140478751464] 
\draw    (804.89,464.98) -- (833.08,464.98) ;
%Shape: Rectangle [id:dp6283534568839406] 
\draw   (33,369.87) -- (336.12,369.87) -- (336.12,498) -- (33,498) -- cycle ;
%Straight Lines [id:da7766228141098565] 
\draw    (425,347) -- (425,432) ;
\draw [shift={(425,344)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Shape: Rectangle [id:dp0677493839993355] 
\draw   (520.12,369.87) -- (828.12,369.87) -- (828.12,498) -- (520.12,498) -- cycle ;
%Shape: Rectangle [id:dp014110378228816445] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (365.5,433) -- (486.5,433) -- (486.5,491) -- (365.5,491) -- cycle ;

%Shape: Rectangle [id:dp8640505621986145] 
\draw  [fill={rgb, 255:red, 144; green, 255; blue, 229 }  ,fill opacity=1 ] (213.49,510.15) -- (335,510.15) -- (335,542) -- (213.49,542) -- cycle ;

%Shape: Rectangle [id:dp11807891437834184] 
\draw  [fill={rgb, 255:red, 144; green, 255; blue, 229 }  ,fill opacity=1 ] (520.49,510.15) -- (642,510.15) -- (642,542) -- (520.49,542) -- cycle ;

%Straight Lines [id:da6023255336667221] 
\draw    (74.14,477.2) -- (74.14,530) ;
%Straight Lines [id:da047541439752831094] 
\draw    (783.02,477.06) -- (783.02,529.87) ;
%Straight Lines [id:da38440122612945915] 
\draw    (74.14,530) -- (215.16,530) ;
\draw [shift={(138.15,530)}, rotate = 0] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Shape: Rectangle [id:dp7774128051215404] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (369.49,510.15) -- (491,510.15) -- (491,542) -- (369.49,542) -- cycle ;
%Straight Lines [id:da048020115234232885] 
\draw    (308,370) -- (336,397) ;
%Straight Lines [id:da22128359563915156] 
\draw    (551.33,370) -- (519.33,398) ;
%Straight Lines [id:da4178126076311651] 
\draw    (427,561) -- (427,584) ;
\draw [shift={(427,558)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da2712874934584891] 
\draw    (427,543) -- (427,558) ;
%Straight Lines [id:da22537158810197067] 
\draw    (377,560) -- (377,583) ;
\draw [shift={(377,557)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da17343167705220275] 
\draw    (377,542) -- (377,557) ;
%Straight Lines [id:da5797829827731849] 
\draw    (473,561) -- (473,584) ;
\draw [shift={(473,558)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da3209997322336591] 
\draw    (473,543) -- (473,558) ;

% Text Node
\draw (147.12,444.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{53.57pt}\setlength\topsep{0pt}
\begin{center}
Random \\Reshuffling
\end{center}

\end{minipage}};
% Text Node
\draw (382,444) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{62.26pt}\setlength\topsep{0pt}
\begin{center}
Richardson\\Extrapolation
\end{center}

\end{minipage}};
% Text Node
\draw (721,118.4) node [anchor=north west][inner sep=0.75pt]    {$\gamma $};
% Text Node
\draw (725,138) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {Step Size\\};
% Text Node
\draw (633.84,444.37) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{53.57pt}\setlength\topsep{0pt}
\begin{center}
Random \\Reshuffling
\end{center}

\end{minipage}};
% Text Node
\draw (107.08,439.73) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{k}^{e}$};
% Text Node
\draw (241.59,438.5) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{k+1}^{e}$};
% Text Node
\draw (300.38,441.53) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{N}^{e}$};
% Text Node
\draw (57.55,441.12) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{0}^{e}$};
% Text Node
\draw (157.77,381.59) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$e\leftarrow e+1$};
% Text Node
\draw (522.12,373.27) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$2\gamma $};
% Text Node
\draw (581.57,440.59) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{k+1}^{e}$};
% Text Node
\draw (733.67,442.41) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{k}^{e}$};
% Text Node
\draw (538.59,442.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{N}^{e}$};
% Text Node
\draw (781.21,443.59) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{0}^{e}$};
% Text Node
\draw (433.38,338.53) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$y^{e} =2x_{( \gamma )}^{e} -x_{( 2\gamma )}^{e}$};
% Text Node
\draw (639.77,380.59) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$e\leftarrow e+1$};
% Text Node
\draw (338.38,444.53) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{( \gamma )}^{e}$};
% Text Node
\draw (490.38,443.53) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{( 2\gamma )}^{e}$};
% Text Node
\draw (223.12,516.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{72.45pt}\setlength\topsep{0pt}
\begin{center}
Pre-Processing
\end{center}

\end{minipage}};
% Text Node
\draw (323.83,369.96) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$\gamma $};
% Text Node
\draw (530.12,516.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{72.45pt}\setlength\topsep{0pt}
\begin{center}
Pre-Processing
\end{center}

\end{minipage}};
% Text Node
\draw (382.12,516.5) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{63.95pt}\setlength\topsep{0pt}
\begin{center}
 \ \ VI Operator
\end{center}

\end{minipage}};
% Text Node
\draw (435,571.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$F( x)$};
% Text Node
\draw (385.38,567.53) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\gamma $};
% Text Node
\draw (367,588) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {Step Size};
% Text Node
\draw (481,570.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{0}$};


\end{tikzpicture}


==> Shuffle_the_Data_arxiv_version_/model_assumptions.tex <==
\section*{Our model's assumptions.}
While variational inequalities provide a unifying language for optimization, learning, and game dynamics, \emph{no single structural assumption can capture the full complexity of all modern nonconvex--nonconcave problems}. From a computational standpoint, even smooth VIs are intractable in full generality---being tightly connected to Nash equilibria~\citep{
papadimitriou2022computational,goldberg2022ppad}, linear complementarity~\citep{ieor2011linear}, and constrained saddle-point problems~\citep{daskalakis2021complexity}. Consequently, much of the theoretical literature adopts \emph{structured} assumptions (strong convexity, quasi-strong monotonicity, quasar or weak convexity, PL/KL conditions, Minty conditions, error bounds, etc.), each expressive in specific regimes but not universal.

Our work is based on \emph{quasi-strong monotonicity} which falls squarely within this class: it captures stabilizing behaviors of many smooth systems, while remaining far more permissive than strong convexity or global monotonicity. At the same time, it is helpful to clarify that this assumption is not meant as a universal model for all adversarial or fully nonconvex--nonconcave settings. Certain modern ML applications---
including GANs, adversarial robustness, and multi-agent RL---can exhibit fundamentally unstable or rotational dynamics~\citep{Jin2020LocalOptimality,Han2023RiemannianMinimax,KimSeo2022SemiImplicit,Bukharin2023RobustMARL}, where even \emph{local} monotonicity surrogates fail. As such, our theoretical guarantees should be viewed as pertaining to regimes where a minimum amount of local structure is present, rather than to the most adversarial or unstructured cases.
\footnote{A complementary and key fact for our setting, established in \citep[Lemma~A.4]{hsieh2019convergence}, is that \emph{any smooth VI operator is locally quasi-strongly monotone in a neighborhood of a regular solution}. Combined with our Markov-chain recurrence result—which ensures that the iterates remain in such neighborhoods with probability~1—this provides a natural and widely adopted stability regime in which the $\RRresh$ and $\RRrom$ debiasing mechanisms are both theoretically justified and practically meaningful.
}

==> Shuffle_the_Data_arxiv_version_/problem_setup.tex <==
% !TEX root = ./iclr2026_conference.tex

\begin{figure}[t]
  \centering
  \resizebox{\textwidth}{!}{\input{algo_figure}}
  \caption{%
    \textbf{Overview of \textup{SGD-}\RRrom$\oplus$\RRresh\ (Algorithm~\ref{alg:rrrom-rrresh}).}
    Two synchronized runs—\textbf{Run~A} (blue, step $\gamma$) and \textbf{Run~B} (orange, step $2\gamma$)—share
    the same random permutation $\omega_k$ at each epoch, producing epoch-end iterates
    $x_k^{[\gamma]}$ and $x_{k}^{[2\gamma]}$. The \RRrom\ outer loop combines them as
    $\hat{x}_{k}=2x_k^{[\gamma]}-x_k^{[2\gamma]}$, canceling the leading
    $\mathcal{O}(\gamma)$ bias term. The resulting asymptotic bias is $\mathcal{O}(\gamma^3)$,
    a strict cubic improvement over either heuristic alone.
  }
  \label{fig:algo_overview}
\end{figure}



\section{Problem setup and assumptions}
\paragraph{Variational inequalities.}  
Let's recall first the basic framework of finite-sum variational inequalities (VIs), which will underlie our analysis. 
Let $X \subseteq \R^d$ be a nonempty closed convex set and $F:\R^d \to \R^d$ a single-valued operator. 
The variational inequality problem $\mathrm{VI}(X,F)$ asks for a point $x^\star \in X$ such that
\begin{equation} \tag{VIP}
    \langle F(x^*), x - x^*\rangle \geq 0, \quad \forall x \in X \label{VIP}
\end{equation}
In our setting, we focus on the unconstrained finite-sum case, i.e. $X=\R^d$ and
\(
F(x) = \frac{1}{n} \sum_{i=0}^{n-1} F_i(x),
\)
respectively, where each $F_i:\R^d \to \R^d$ typically represents the gradient of a loss function for a data point in some dataset $\mathcal{D}$.
To build intuition, we illustrate the framework through a few canonical examples below:\\
\textbf{Example 2.1: Solving Non-linear equations.} A solution $x^*$ to the \eqref{VIP} corresponds to a root of the equation $F(x) = \textbf{0}$. Therefore, we can cast any non-linear equation as a specific instantiation of the Variational Inequality framework. Well-known examples include the Navier-Stokes equations in computational dynamics \citep{hao2021gradient}. \\
\textbf{Example 2.2: Empirical Risk Minimization.} For any $\mathcal{C}^1-$smooth loss function $\ell:\R^d \rightarrow \R$, a solution $x^*$ to the \eqref{VIP} with $F(x) = \nabla \ell(x)$ is a critical point (KKT solution) to the associated empirical risk minimization problem, consisting the cornerstone of machine learning objectives.\\
\textbf{Example 2.3: Nash Equilibria \& Saddle-point Problems.}
Consider $N$ players, each having an action set in $\R^d$ and a convex cost function $c_i: \R^d\rightarrow \R$. A Nash Equilibrium \eqref{NE} is a joint-action profile $x^* = (x^*_i)_{i=1}^N$ that satisfies
\begin{equation}\tag{NE}
    c_i(x^*) \leq c_i(x_i; x^*_{-i}), \quad \forall i, x_i \in \R^d \label{NE}.
\end{equation}
For convex cost functions $c_i: \R^d \rightarrow \R$, a \eqref{NE} coincides with the solution of a \eqref{VIP} with operator $F(x) = \left(\nabla_{x_{i}} c_i(x)\right)_{i=1}^N$. 
In the particular case of two players and a (quasi) convex-concave objective $\mathcal{L}: \R^d \times \R^d \rightarrow \R$, the solution $x^* = (x_1^*, x_2^*)$ to the \eqref{VIP} with $F(x) = (\nabla \mathcal{L}(x), - \nabla \mathcal{L}(x))$ is a saddle point of $\mathcal{L}$ satisfying
\begin{equation*}
    \mathcal{L}(x^*_1, x_2) \leq \mathcal{L}(x^*_1, x^*_2) \leq \mathcal{L}(x_1, x^*_2), \quad \forall x_1, x_2 \in \R^d. \nonumber
\end{equation*}
Saddle-point problems and applications of \eqref{NE} are ubiquitous, from training Generative Adversarial Networks (GANs) to multi-agent reinforcement learning and auction/bandit problems \citep{daskalakis2017training, zhang2021multi, pfau2016connecting}.

\paragraph{Blanket assumptions.}  
We now state the standing assumptions for our analysis, beginning with the existence of a solution $x^\star$ to \eqref{VIP}.
\begin{assumption} \label{assumt: sol_set_non_empty}
    The solution set $\mathcal{X}^*$ of \eqref{VIP} is nonempty and there exists $x^* \in \mathcal{X}^*, R \in \mathbb{R} $ such that $\|x^*\|_2 \leq R$.
\end{assumption}
The next assumption introduces the class of operators $F$ of the associated \eqref{VIP} for which our stochastic gradient algorithms will be analyzed.

\noindent
\begin{minipage}[t]{0.56\textwidth}
\vspace{0pt}
\begin{assumption}[$\lambda$-weak $\mu$-quasi strong monotonicity] \label{assumpt: weak_quasi_strong_monotonicity}
    The operator $F$ is $\lambda$-weak $\mu$-quasi strongly monotone, i.e. there exist $\lambda \geq 0, \mu > 0$ such that for some $x^*\in\mathcal{X}^*$ it holds that
    \begin{eqnarray}
        \langle F(x), x - x^*\rangle &\geq& \mu \|x - x^*\|^2 - \lambda, \quad \forall x \in \mathbb{R}^d .
    \end{eqnarray}
\end{assumption}

Assumption~\ref{assumpt: weak_quasi_strong_monotonicity} for $\lambda = 0$ coincides with the well-known notions of quasi-strong monotonicity \citep{loizou2020stochastic}, strong stability condition \citep{mertikopoulos2019learning}, and strongly coherent VIPs \citep{song2020optimistic} in the optimization literature. It can be seen as a relaxation of the classical notion of strong monotonicity/convexity, which requires
$\langle F(x) - F(x'),\, x - x'\rangle \geq \mu \|x - x'\|^2$ for all $x,x'\in \R^d$.
For $\lambda > 0$, Assumption~\ref{assumpt: weak_quasi_strong_monotonicity} represents a further relaxation, motivated by dissipative dynamical systems and weakly convex optimization \citep{raginsky2017non, erdogdu2018global}, and it encompasses non-monotone games as well as a variety of problems in statistical learning theory \citep{tan2023online}.
\end{minipage}%
\hfill%
\begin{minipage}[t]{0.40\textwidth}
\vspace{0pt}
\centering
\includegraphics[width=\linewidth]{./figures/weakly.png}
\captionof{figure}{A simple example satisfying
    Assumption~\ref{assumpt: weak_quasi_strong_monotonicity}:
    $f(x,y)=(x^2+7\sin x)+xy-(y^2-7\cos y)$,
    with $(\mu,\lambda)=(1,25)$.}
\label{fig:weak_example}
\end{minipage}

A common assumption in the literature of smooth optimization that we will utilize is that the operators in the finite-sum structure of the \eqref{VIP} are Lipschitz continuous.%\vspace{-4em}


\begin{assumption}[Lipschitz continuity]\label{assumpt: lipschitz}
Each $F_i$ is $L_i$-Lipschitz:
\[
\|F_i(x_1)-F_i(x_2)\| \le L_i\|x_1-x_2\|,
\qquad \forall x_1,x_2\in\R^d,\; i\in[n],
\]
with $L_{\max}=\max_{i\in[n]}L_i$.
\end{assumption}

Unlike standard analyses assuming unbiased oracles with bounded variance, e.g., \citep{loizou2021stochastic,hsieh2019convergence,lin2020finite,mishchenko2020revisiting},
random reshuffling induces bias via inter-step dependence.  
Such conditions may fail even for simple quadratics.  
Instead, we work directly with Lipschitz continuity and impose only a mild moment bound:
\begin{assumption}[Bounded moments at the solution]\label{assumpt: 4th-moment bounded}
At some $x^*\in\mathcal{X}^*$, the oracle values have finite second and fourth moments:
\[
\sigma_*^2:=\frac{1}{n}\sum_{i=1}^n\|F_i(x^*)\|^2<\infty,
\qquad 
\sigma_*^4:=\frac{1}{n}\sum_{i=1}^n\|F_i(x^*)\|^4<\infty.
\]
\end{assumption}

Assumption~\ref{assumpt: 4th-moment bounded} is mild: it does not require global boundedness of gradients, but only that the oracle values $F_i(x^*)$ admit finite second and fourth moments at the solution.  
Building on this, we extend the variance bound of~\citet[Prop.~A.2, p.~16]{emmanouilidis2024stochastic} to higher-order moments.  
\begin{proposition}\label{prop}
Let Assumptions~\ref{assumt: sol_set_non_empty}--\ref{assumpt: lipschitz} hold. Then, for any $x\in\R^d$ it holds that
\begin{align*}
&\text{(i)}~~\frac1n\sum_{i=1}^n \|F_i(x)-F(x)\|^2
\;\le\;
\frac2n\sum_{i=1}^n L_i^2\|x-x^*\|^2 \;+\; 2\sigma_*^2,\\[0.5em]
&\text{(ii)}~~\frac1n\sum_{i=1}^n \|F_i(x)-F(x)\|^4
\;\le\;
\frac{128}{n}\sum_{i=1}^n L_i^4 \|x-x^*\|^4 \;+\; 128\sigma_*^4.
\end{align*}
\end{proposition}
Having introduced the necessary assumptions, we, next, provide the proposed algorithm that will achieve the higher order bias refinement in our results.

\bluecomment{
\section{The algorithmic framework}  
While there are many conceivable ways to interleave \RRrom\ and \RRresh, both intra- and inter-epoch, we adopt the most natural and practically motivated design. In modern pipelines, \RRresh\ is the workhorse at the low-level training stage, while \RRrom\ is often employed as a black-box refinement at a higher level, allowing parallelization and modular integration. Accordingly, we study stochastic gradient algorithms that sample via random reshuffling to generate stochastic oracles of gradients/operators. At the start of each epoch $k>0$, a random permutation $\omega_k$ of $[n]$ is drawn, prescribing the order in which data points are processed. The algorithm then performs the classical SGD update:
\begin{equation}\tag{SGD-\RRrom$\oplus$\RRresh (inner-loop)}
\footnotesize
    x_k^{i+1} = x_k^i - \gamma \,\mathrm{PreProcess}\big[\mathrm{StochOracle}(x^i_k; \omega_k^i)\big],
    \label{SGD-4R1}
\end{equation}

where $\mathrm{StochOracle}(x^i_k; \omega_k^i)$ denotes either the stochastic gradient (in minimization problems) or the operator value $F_{\omega_k^i}(x^i_k)$ (in the general VI case), indexed by the $\omega_k^i$ data point and $\mathrm{PreProcess}[\cdot]$ is a preprocessing routine implementing calibrated Gaussian smoothing to the input. Then, the final iterate of each epoch becomes the starting point of the next, and the procedure repeats.

\begin{algorithm}[ht]
\caption{\textsc{SGD--\RRrom$\oplus$\RRresh}}
\label{alg:rrrom-rrresh}
\begin{algorithmic}[1]
\footnotesize
\Require Initial point $x_0\in\R^d$; step size $\gamma>0$; epochs $I$; dataset size $n$;
\Statex \hspace{\algorithmicindent} \textsc{StochOracle}$(x;i)$ returns $F_i(x)$ (minimization) or operator value (VI);
\Statex \hspace{\algorithmicindent} \textsc{PreProcess}$(g;i)$ adds calibrated Gaussian smoothing on $g$ (e.g., $\;\;\noise_k \sim \mathcal{N}(0,\, \gamma^2 n \sigma_*^2 I)$).
\For{$k=0,1,\dots,I-1$} \Comment{epoch $k$}
  \For{$\eta=\gamma,2\gamma$}   \Comment{Parallel iterations with two step-sizes}
  \State Draw a random permutation $\omega_k$ of $[n]$
  \For{$i=0,1,\dots,n-1$} \Comment{inner loop (reshuffled pass)}
    \State $x^{i+1}_{k,[\eta]}   \gets x^{i}_{k,[\eta]}   - \eta\, \textsc{PreProcess}( \textsc{StochOracle}(x^{i}_{k,[\eta]},  \omega_k[i]))$
  \EndFor
    \State $x^{0}_{k+1,[\eta]} \gets x^{n}_{k,[\eta]}$ \Comment{baseline next-start (used for analysis)}%; output uses $\hat{x}$}
  \EndFor
  \State $\hat{x}_{k+1} \gets 2\,x^{n}_{k,[\gamma]} - x^{n}_{k,[2\gamma]}$   \Comment{outer loop ( extrapolation at epoch end)}
  \Statex \ \ \ \  \ \ \ \ \ \ \ \ OR
  \State $\hat{x}_{k+1} \gets (2\,\sum_{m\in[k]}x^{n}_{k,[\gamma]} - x^{n}_{m,[2\gamma]})/k$ \Comment{Alternative: ( extrapolation at epoch's averages)}
\EndFor
\State \textbf{return} $\hat{x}_{I}$ \Comment{(optionally average $\{\hat{x}_k\}$ across epochs)}
\end{algorithmic}
\end{algorithm}

\emph{On the necessity of smoothing.}
A key challenge with reshuffling is that, after one epoch, the cumulative gradient estimator is biased, unlike sampling with replacement, which is unbiased and analytically simpler. The induced noise is also discrete, tied to permutations. 
To handle this, we introduce a calibrated Gaussian perturbation that smooths the discrete reshuffling noise into a well-behaved proxy while preserving variance, moments, and bias order. In practice, the perturbation has negligible effect across datasets; clarifying its precise dependence on dataset size is an interesting direction for future work. For completeness, the supplement also includes a brief sketch showing how our results extend even without this step.
Finally, at the end of each epoch we apply \RRrom, yielding the extrapolated update:
\begin{equation}\tag{SGD-\RRrom$\oplus$\RRresh (outer-loop)}
    \hat{x}^N_{I+1} = 2\,x^{N}_{I,[\gamma]} - x^{N}_{I,[2\gamma]}\,.
    \label{SGD-4R2}
\end{equation}
In Section~\ref{sec:results}, we prove that this combination achieves a provable $\mathcal{O}(\gamma^3)$ bias— to the best of our knowledge, the first such result.
}

==> Shuffle_the_Data_arxiv_version_/results.tex <==
% !TEX root = ./iclr2026_conference.tex
\bluecomment{\section{Theoretical Guarantees}\label{sec:results}}
\kostas{We present the theoretical guarantees for the synergy of both heuristics in our algorithm, establishing a cubic refinement in the bias attained. We start by analyzing the \RRresh\ component (inner loop of Algorithm~\ref{alg:rrrom-rrresh}), which serves as the basis for performing \RRrom\ (outer loop of Algorithm~\ref{alg:rrrom-rrresh}) on the produced iterates and describe the interplay of both heuristics in the bias of Algorithm~\ref{alg:rrrom-rrresh}.}

\subsection{Convergence Guarantees for \RRresh} 
% \vspace{-0.75em}
\kostas{Our first result concerns the convergence of the \RRresh\ component for $\lambda$-weak $\mu$-quasi strongly monotone VIPs. More specifically, in order to effectively utilize Markov Chain tools we study the \RRresh\ variant under preprocessing perturbations\footnote{Empirically, for sufficiently large datasets 
the effect of discrete noise in smooth problems is negligible, making the preprocessing 
step unnecessary. A detailed study of this effect lies beyond the scope of this paper, 
whose focus is instead the first systematic treatment of the interaction between Random reshuffling and 
Richardson extrapolation.} (inner loop of Algorithm~\ref{alg:rrrom-rrresh}), attributing for simplicity of exposition of our results the name Perturbed SGD–\RRresh. }

\begin{theorem}\label{thm: convergence_rate}
    Let Assumptions~\ref{assumt: sol_set_non_empty}-\ref{assumpt: lipschitz} hold. If $\gamma \leq \gamma_{max}$, 
    then the iterates of {Perturbed SGD–\RRresh} satisfy
    \begin{eqnarray}
        \ex\left[\|x_{k+1}^0 - x_*\|^2\right] &\leq& \left(1 - \frac{\gamma  n\mu}{2}\right)^{k+1} \|x^0_0 - x^*\|^2 + \frac{8 n \gamma^2 L_{max}^2}{\mu^2} \sigma_*^2 + \frac{8\lambda}{\mu} \nonumber
    \end{eqnarray}
   where  $\sigma_*^2 = \frac{1}{n} \sum_{i=0}^{n-1} \|F_i(x^*)\|^2$ and $\gamma_{max} = \min\left\{\frac{1}{3nL_{max}}, \frac{\sqrt{1+6 \mu^2 L_{max}^2} -1}{12nL_{max}^2}\right\}$.
\end{theorem}
% \vspace{-0.75em}
\begin{draftremark}
Theorem~\ref{thm: convergence_rate} establishes exponential convergence up to a bias of $\mathcal{O}(\gamma^2\sigma_*^2 + \tfrac{\lambda}{\mu})$, where the $\tfrac{8\lambda}{\mu}$ term is inherent \citep{yu2021analysis}. For fair comparison we focus on the quasi-strongly monotone case ($\lambda=0$), which already generalizes strong convexity. Our rate recovers known results for strongly monotone operators \citep{das2022sampling,emmanouilidis2024stochastic} and extends them to weak monotonicity.
In this regime, reshuffling attains a much smaller bias than the $\mathcal{O}(\gamma\sigma_*^2)$ of with-replacement SGD \citep{loizou2020stochastic,gower2019sgd}, converging to a tighter neighborhood. This sharper bias also yields faster accuracy rates: with $\gamma = 1/(nK)$, with-replacement SGD reaches $\mathcal{O}(1/(nK))$ accuracy \citep{das2022sampling,mishchenko2020random}, while reshuffling accelerates to $\mathcal{O}(1/(nK^2))$, a further  support for its empirical success.
\end{draftremark}


\begin{table}[t]
\centering
\scalebox{0.92}{
\footnotesize
\begin{tabular}{lcc}
\toprule
\textbf{Aspect} & \textbf{\cite{emmanouilidis2024stochastic}} & \textbf{Our work} \\
\midrule

Baseline Algorithm & \textbf{SEG} & \textbf{SGDA} \\[2pt]

Model Assumptions (Smoothness) &
$F_i$--$L_i$ Lipschitz &
$F_i$--$L_i$ Lipschitz
\\[2pt]

Model Assumptions (Drift) &
$F$ $\mu$--strongly monotone &
$F$ \emph{quasi}--strongly monotone
\\[2pt]

Main heuristic & \textbf{\RRresh\ only} & \textbf{\RRresh\ $\oplus$ \RRrom} \\[2pt]

Asymptotic Bias order & $\mathcal{O}(\gamma + \gamma^3)$ & $\mathcal{O}(\gamma^3)$ \\[2pt]

Asymptotic MSE order & $\mathcal{O}(\gamma^2)$ & $\mathcal{O}(\gamma^2)$ \\[2pt]

Condition number & \textbf{Worse than vanilla-SEG} & \textbf{Same as vanilla-SGDA} \\[2pt]

Mechanism & EG-structure + $\RRresh$ & Bias cancellation ($\RRresh \oplus \RRrom$) \\
\bottomrule
\end{tabular}
} % end scalebox
\caption{Summary of key differences between \cite{emmanouilidis2024stochastic} and our results.}
\label{tab:comparison}

\end{table}

In the sequel, we view the algorithmic trajectory through the prism of Markov chain theory. This perspective enables a finer dissection of the reshuffling bias and, mutatis mutandis, equips us with the machinery to construct consistent estimators for performance statistics. The Markovian framework arises naturally, as the method progresses from $x_k$ to $x_{k+1}$ in a state-dependent fashion. The connection between stochastic approximation and Markov processes—traced back to early works such as \cite{robbins1951stochastic,pflug1986stochastic}—has fueled a rich literature for algorithms with unbiased oracles. Random reshuffling, however, generates systematically biased oracles, necessitating a genuine departure from this canonical line of analysis.

For readers accustomed only to classical finite-state Markov chains, the transition mechanism is usually represented by a directed graph with fixed transition probabilities.
In our setting, the analogue is the transition kernel
$P(x,A)=\Pr\!\big[x_{\text{next}}\in A \,\mid\, x_{\text{now}}=x\big], A\in\mathcal{B}(\R^d)$,
where $\mathcal{B}(\R^d)$ denotes the Borel sets of $\R^d$.
As in the finite-state case, it is highly desirable that this kernel remain invariant over time—this is the property of time-homogeneity.\footnote{If time-homogeneity fails, a process can be still Markovian in the sense that the future depends only on the present, but its statistical regularity vary with time, complicating both analysis and long-run guarantees.}

At the step level, reshuffling destroys homogeneity: the transition kernel varies with the permutation index, making the process non-stationary.
Fortunately, this irregularity vanishes at the epoch scale:\begin{center}
\emph{``After one reshuffled pass, the law of the next iterate depends only on the epoch’s starting point and the drawn permutation, but not its position within the permutation.''}\end{center}
Thus, the sequence of epoch-level iterates $(x^{[0]}_{{k}})_{_{{k}\ge0}}$ forms a bona fide time-homogeneous Markov chain,  forming the basis for the asymptotic analysis of the \RRrom\ extrapolation component \footnote{On the augmented space $\R^d\times\mathfrak{S}_n$, the chain $((x_k,\omega_k))_{k\ge0}$ is also time-homogeneous with kernel
\(
K\big((x,\omega),A\times B\big)
=\int_A \phi\big(y;H(x,\omega),\Sigma I_d\big)\,dy\cdot \frac{|B|}{n!}.
\)
The above formulation is convenient for verifying Lyapunov–Foster and minorization criteria, since the coupling with uniform perturbation remains independent.}

\begin{lemma}[Epoch-level homogeneity and kernel]\label{lem:epoch-homog}
Fix $\gamma>0$ and $n\in\mathbb{N}$. Then the \emph{Perturbed SGD-\RRresh\ } can be described at each epoch $k$ as:
\emph{Draw $\omega_k$ uniformly from $\mathfrak{S}_n$ and set}
\[
x_{k+1}
\;=\;
H(x_k,\omega_k)\;+\;U_k, 
\quad U_k\sim \mathcal N(0,\Sigma),
\]
where $H(x,\omega)$ denotes the endpoint of one reshuffled pass started at $x$ with permutation $\omega$ (i.e., the map induced by $n$ inner updates with step size $\gamma$). Then $(x_k)_{k\ge 0}$ is a time-homogeneous Markov chain on $\R^d$ with transition kernel
\[
P(x,A)
\;=\;
\frac{1}{n!}\sum_{\omega\in\mathfrak{S}_n}
\int_A \phi\!\big(y;\,H(x,\omega),\,\Sigma \big)\,dy,
\qquad A\in\mathcal{B}(\R^d),
\]
where $\phi(\cdot;m,\Sigma )$ is the $d$-variate Gaussian density with mean $m$ and covariance $\Sigma$.
\end{lemma}

By verifying irreducibility, aperiodicity, and \emph{positive Harris recurrence} \citep{meyn2012markov}, we establish a unique invariant distribution $\pi_\gamma$, geometric convergence in total variation to it, and concentration of scalar observables (admissible test functions) around $x^*$.
\begin{theorem}\label{thm: efficient_stats}
Under Assumptions~\ref{assumt: sol_set_non_empty}--\ref{assumpt: lipschitz}, run Perturbed SGD-\RRresh with $\gamma\le\gamma_{\max}$. Then $(x_k)_{k\ge0}$ admits a unique stationary distribution $\pi_\gamma\in\mathcal P_2(\R^d)$, and additionally:
\begin{align*}
&\text{(i)}~~ |\ex[\ell(x_k)]-\ex_{x\sim\pi_\gamma}[\ell(x)]|\;\le\;c(1-\rho)^k 
&& \forall \ell:|\ell(x)|\le L_\ell(1+\|x\|), \\
&\text{(ii)}~~ |\ex_{x\sim\pi_\gamma}[\ell(x)]-\ell(x^*)|\;\le\;L_\ell\sqrt{C} 
&& \forall \ell:  L_\ell-\text{Lipschitz functions},
\end{align*}
for some $c<\infty$, $\rho\in(0,1)$, $C=\Theta(\mathrm{MSE}(\texttt{SGD}-{\RRresh}))$ and $\gamma_{\max}$ defined in Theorem~\ref{thm: convergence_rate}%$\gamma_{\max}=\gammaub$
\end{theorem}
\begin{draftremark}
Item (i) of Theorem~\ref{thm: efficient_stats} shows that Perturbed SGD-\RRresh converges geometrically in total variation to $\pi_\gamma$.
Item (ii) bounds the gap between the expectation of a measurement under $\pi_\gamma$ and its value at the solution $x^*$. Intuitively, if the method converged exactly to $x^*$, these expectations would coincide.
\end{draftremark}

The result of Theorem~\ref{thm: efficient_stats} follows from a Foster–Lyapunov drift condition combined with a minorization argument, showing that the induced Markov chain satisfies the standard ergodicity criteria in the spirit of \citet{yu2021analysis,vlatakis2024stochastic}.
Beyond geometric ergodicity, one may also ask whether the chain admits asymptotic statistical estimation of functionals of its trajectory. By invoking the Birkhoff--Khinchin ergodic theorem for continuous-state Markov chains, we establish both a Law of Large Numbers (LLN) and a Central Limit Theorem (CLT) for empirical averages of test functions evaluated along the epoch iterates.

\begin{theorem}[LLN and CLT for Perturbed SGD--\RRresh]\label{thm: LLN_CLT_res} 
Suppose Assumptions~\ref{assumt: sol_set_non_empty}--\ref{assumpt: lipschitz} hold and run Perturbed SGD--\RRresh\ with $\gamma \le \gamma_{\max}$, (cf.\ Theorem~\ref{thm: convergence_rate}). Let $\ell:\R^d\to\R$ be any test function such that $|\ell(x)|\le L_\ell(1+\|x\|^2)$ and $\ex_{x\sim\pi_\gamma}[\ell(x)]<\infty$.
Then for the epoch-level iterates it holds that:
\begin{eqnarray}
   &&\underbrace{\frac{1}{T}\sum_{t=0}^{T-1}\ell(x_t) 
  \;\xrightarrow{\text{a.s.}}\; \ex_{x\sim\pi_\gamma}[\ell(x)]}_{\text{(LLN)}}\qquad
 \underbrace{T^{-1/2}\sum_{t=0}^{T-1}\!\Big(\ell(x_t)-\ex_{x\sim\pi_\gamma}[\ell(x)]\Big) 
  \;\xrightarrow{d}\; \mathcal N(0,\sigma^2_{\pi_\gamma}(\ell))}_{\text{(CLT)}},\nonumber
\end{eqnarray}
where $\sigma^2_{\pi_\gamma}(\ell)=\lim_{T\to\infty}\tfrac{1}{T}\ex_{\pi_\gamma}[S_T^2]$ and $S_T^2=\sum_{t=0}^{T-1}\big(\ell(x_t)-\ex_{x\sim\pi_\gamma}[\ell(x)]\big)^2$.

\end{theorem}

\subsection{Convergence Guarantees for \RRrom$\oplus$\RRresh}% The Outer loop
Having established the role of \RRresh\ within stochastic algorithms, we now examine its interplay with \RRrom\ and the effect of combining these heuristics on the bias term.
The previous results hold for the full class of weakly quasi-strongly monotone problems with $\lambda>0$.  
To sharpen our understanding, we focus on the quasi-strongly monotone case ($\lambda=0$ in Assumption~\ref{assumpt: weak_quasi_strong_monotonicity}), which already covers a broad range of non-monotone regimes \citep{loizou2020stochastic}.  
A key step in our analysis is to bound higher-order moments of the deviation between \RRresh\ iterates and the solution of \eqref{VIP}, thereby showing that the bias of Perturbed SGD--\RRresh\ is linear in the step size with quadratic corrections. 


Technically, our analysis relies on two delicate ingredients that go beyond straightforward generalizations.  
(i) A \emph{spectral study of the full-pass operator} (Lemma~\ref{lemma: eigenvalues_operator}), which approximates the underlying map $F$ of the VIP.  
This connection between \RRresh\ and the multi-step extragradient literature may be of independent interest, but its proof requires a nontrivial handling of spectral properties across reshuffled passes.  
(ii) A \emph{combinatorial lemma} (Lemma~\ref{lemma: 4th-order-property}) that bounds fourth order moments of finite-sum subsets of vectors.  
While reminiscent of \citet[ Lemma~1, Sec.~7]{mishchenko2020revisiting}, our result demands substantially more intricate manipulations to accommodate the dependencies introduced by sampling without replacement.
% \vspace{-0.5em}
\begin{lemma}\label{lem: rr_1}
Let $\lambda=0$ and Assumptions~\ref{assumt: sol_set_non_empty}--\ref{assumpt: 4th-moment bounded} hold.  
If $\gamma\le\gamma_{\max}$ (cf.\  Lemma~\ref{lemma strongly monotone 4th-moment}), then
\[
\mathrm{bias}(\texttt{Perturbed SGD-\RRresh})
=\limsup_{k\to\infty}\|\ex[x_k]-x^*\|
= C(x^*)\gamma+\mathcal{O}(\gamma^3).
\]
\end{lemma}
% \vspace{-0.5em}

\begin{draftremark}
For classical \texttt{SGD}, the bias takes the form 
$\mathrm{bias}(\texttt{SGD})=C(x^*)\gamma+\mathcal{O}(\gamma^{1.5})$ \citep{dieuleveut2020bridging}.  
Hence, while \RRresh\ retains the same first-order term, it improves the higher-order contribution and simultaneously yields sharper mean-squared error guarantees.
\end{draftremark}
% \vspace{-0.5em}
\newpage
Building on this fact, we construct a refined trajectory via the debiasing scheme \RRrom.  
Our final result shows that the combined scheme attains exponentially fast a provable asymptotic $\mathcal{O}(\gamma^3)$ bias:
% \vspace{-0.5em}

\begin{theorem}\label{thm: rr_1_rr_2}
   Under the assumptions of Lemma~\ref{lem: rr_1}, Algorithm~\ref{alg:rrrom-rrresh} output satisfies
   \[\begin{aligned}
   &\text{Last-iterate version (line 9):} 
   && \|\ex[x_k]-x^*\|\;\le\;c(1-\rho)^k+\mathcal{O}(\gamma^3), \\[0.5em]
   &\text{Averaged-iterate version (line 10):} 
   && \Biggl\|\ex\!\left[\tfrac{1}{k}\sum_{m=1}^k x_m\right]-x^*\Biggr\|\;\le\;\tfrac{c/\rho}{k}+\mathcal{O}(\gamma^3).
   \end{aligned}\]
   and the attained MSE is bounded by
   \begin{eqnarray}
       \ex\left[\|x_k - x^*\|^2\right] &\leq& c' (1-\rho')^k + \mathcal{O}\left(\gamma^2\right) \nonumber
   \end{eqnarray}
   where $\rho, \rho' \in(0,1),\;c, c' <\infty$.
\end{theorem}
% \vspace{-0.5em}

\begin{draftremark}
Although the \emph{last-iterate} estimator is often preferred in theory, in practice a trade-off emerges vs \emph{ergodic-average}: full-epoch or tailed averaging (the Polyak--Ruppert scheme~\citep{polyak1992acceleration}) achieves improved variance properties, asymptotically captured by Theorem~\ref{thm: LLN_CLT_res}.
\end{draftremark}



==> Shuffle_the_Data_arxiv_version_/rr_intuition_figure.tex <==
% rr_intuition_figure.tex — v14
\begin{tikzpicture}[
    >=stealth,
    every node/.style={font=\small},
    dot/.style={circle,fill,inner sep=2.8pt},
    lbl/.style={inner sep=6pt, rounded corners=4pt, thick},
]
  \colorlet{colA}{blue!75!black}
  \colorlet{colB}{orange!85!black}
  \colorlet{colR}{red!60!black}
  \definecolor{darkgreen}{RGB}{80,160,10}

  \def\yB{4.20}
  \def\yA{2.00}
  \def\yMid{3.10}
  \def\yE{0.00}
  \def\xT{8.0}
  \def\xRul{9.2}

  % ── Asymptote dashed lines ───────────────────────────────────────
  \draw[colB, densely dashed, opacity=0.40, thin] (0,\yB) -- (\xRul+0.3,\yB);
  \draw[colA, densely dashed, opacity=0.40, thin] (0,\yA) -- (\xRul+0.3,\yA);
  \draw[gray!30, densely dashed, thin] (0,\yE) -- (\xRul+5.5,\yE)
    node[right, gray!45, font=\small] {$x^*$};

  % ── Funnels: manually defined polygons that CONTAIN the trajectories
  \fill[colB, opacity=0.10]
    (0,6.15) .. controls (2,5.52) and (4,4.92) .. (6,4.63) -- (\xT,4.48)
    -- (\xT,3.92) -- (6,4.07) .. controls (4,4.18) and (2,4.28) .. (0,4.85)
    -- cycle;

  \fill[colA, opacity=0.12]
    (0,-0.05) .. controls (2,1.45) and (4,1.85) .. (6,1.92) -- (\xT,2.22)
    -- (\xT,1.78) -- (6,1.48) .. controls (4,0.95) and (2,0.15) .. (0,-1.35)
    -- cycle;

  % ── Trajectories ─────────────────────────────────────────────────
  \draw[colA, line width=1.9pt, ->]
    plot[smooth,tension=0.55] coordinates
      {(0,-0.7)(2,0.8)(4,1.4)(6,1.7)(\xT,\yA)};
  \draw[colB, line width=1.9pt, ->]
    plot[smooth,tension=0.55] coordinates
      {(0,5.5)(2,4.9)(4,4.55)(6,4.35)(\xT,\yB)};

  % ── Faint sphere halos (before dots) ─────────────────────────────
  \node[circle, fill=colB, fill opacity=0.13, draw=colB, draw opacity=0.22,
        inner sep=22pt] at (\xT,\yB) {};
  \node[circle, fill=colA, fill opacity=0.13, draw=colA, draw opacity=0.22,
        inner sep=22pt] at (\xT,\yA) {};
  \node[circle, fill=black, fill opacity=0.10, draw=black, draw opacity=0.18,
        inner sep=11pt] at (\xT+1.3,\yMid) {};

  % ── Terminal dots ────────────────────────────────────────────────
  \node[dot,colA] (zA) at (\xT,\yA) {};
  \node[dot,colB] (zB) at (\xT,\yB) {};
  \node[colA, left=12pt, font=\small\itshape] at (zA) {$x^{k+2}_{\gamma}$};
  \node[colB, left=12pt, font=\small\itshape] at (zB) {$x^{k+2}_{2\gamma}$};

  % ── Extrapolated dot ─────────────────────────────────────────────
  \node[dot,black,inner sep=2.8pt] (xhat) at (\xT+1.3,\yMid) {};
  \node[black, above=5pt, font=\small\bfseries] at (xhat) {$\hat{x}^{k+2}$};

  % ── Run labels ───────────────────────────────────────────────────
  \node[colA, draw=colA, fill=blue!5, lbl] at (1.8,-1.70)
    {\textbf{Run A}\enspace(step $\gamma$)};
  \node[colB, draw=colB, fill=orange!5, lbl] at (1.8, 6.4)
    {\textbf{Run B}\enspace(step $2\gamma$)};

  % ── Bias annotation boxes (inside plot) ──────────────────────────
  \node[colA, draw=colA, fill=blue!4, lbl] at (4.2, 0.45)
    {$\mathrm{Bias}=A\cdot\gamma+\mathcal{O}(\gamma^3)$};
  \node[colB, draw=colB, fill=orange!4, lbl] at (4.2, 5.60)
    {$\mathrm{Bias}=A\cdot(2\gamma)+\mathcal{O}(\gamma^3)$};

  % ── Epoch k ──────────────────────────────────────────────────────
  \draw[->, darkgreen, line width=1.5pt]
    (-0.2,-2.30) -- (\xT+0.3,-2.30);
  \node[darkgreen, right=5pt, font=\small\bfseries]
    at (\xT+0.3,-2.30) {Epoch $k$};

\end{tikzpicture}

==> Shuffle_the_Data_arxiv_version_/titles.tex <==
% !TEX root = ./iclr2026_conference.tex


% \title{Extrapolate the Past, Reshuffle the Future: Bias-Reducing Heuristics in Unity
% }

 % \title{When Reshuffling Meets Extrapolation: Two Heuristics are Better than One in Optimization}

% \title{  Reshuffling Meets Richardson Extrapolation: A Bias-Driven Route to Faster Convergence in VIs.}

% \title{On the Synergy of  Reshuffling and Richardson Extrapolation in  Variational Inequalities}

% \title{Composing Bias Improvements: Two Heuristics, One Accelerated Algorithm}

% \title{Bias-Driven Optimization Heuristics in Unity\\ Reshuffling Meets Richardson Extrapolation
% }

% \title{When Reshuffling Meets Extrapolation: Two Heuristics are Better than One in Optimization}


% \title{Improved Bias Reduction in Optimization: Reshuffling and Extrapolation in Action}

% \title{Bias-Driven Acceleration in VIs: Reshuffling Meets Richardson Extrapolation
% }


% \title{Two Heuristics Are Better than One: Accelerating Gradient Methods in  VIs}


% \title{Shuffling the Data, Stretching the Step-Size: Compositional Bias Reduction in Finite-Sum VIs
% }


% \title{Shuffling the Data, Stretching the Step-Size: Multiplying the Gains  in Finite-Sum Optimization
% }

% \title{Composing Bias-Reducing Heuristics: Reshuffling and Extrapolation Yield $\mathcal{O}({\gamma}^3)$ Bias}

% \title{Synergistic Bias Reduction: How Reshuffling and Extrapolation Accelerate Together in VIs}


% \title{Shuffling the Data, Extrapolating the Step: Two Heuristics, One Accelerated Algorithm}

% \title{Shuffling the Data, Extrapolating the Steps
% When Two Heuristics are Better than One\\
% }
% \title{Shuffling the Data, Extrapolating the Steps
% Cubic Acceleration in Stochastic Optimization
% }

% \title{Improved Bias of Extrapolated Shuffling Gradient Methods for Variational Inequalities}


% \title{When Bias Reductions Multiply: From Simple Heuristics to $\mathcal{O}({\gamma}^3)$ Bias}

% \title{Shuffling the Data, Extrapolating the Steps: Compositional Bias Reduction in Finite-Sums}

% \title{Shuffling the Data, Stretching the Step-Size: Provable Compositional Bias Reduction in VIs }

% \title{Shuffling the Data, Stretching the Step-Size: Compositional Bias Reduction in VIs is Possible }

% \title{Reshuffling Meets Richardson Extrapolation: A Bias-Driven Route to Faster Convergence}
% \title{Reshuffling Meets Richardson Extrapolation: Compositional Bias-Driven Acceleration in VIs}



% Kostas' titles shortlist
% \title{Shuffling the Data, Stretching the Step-Size: Compositional Bias-Driven Acceleration in VIs}
% \title{Reshuffling Meets Richardson Extrapolation: A Bias-Driven Route to Faster Convergence in VIs.}
%\title{Shuffling the Data, Extrapolating the Step: Two Heuristics, One Accelerated Algorithm}
 %\title{Shuffling the Data, Stretching the Step-Size:  A Bias-Driven Route to Faster Convergence }
 %\title{Debiasing Stochastic Gradient Methods: SGD-4R\\The Synergy of Reshuffling and  Extrapolation }
%% \title{Shuffling the Data, Stretching the Step-Size: Debiasing Stochastic Gradient Methods }
%  \title{Shuffling the Data, Stretching the Step-Size: A Sub-cubic Bias SGD Method }
%  \title{Beyond Linear Bias: The Synergy of Reshuffling and Richardson Extrapolation }
%  \title{Reshuffling meets Richardson:  Beyond Linear Bias SGD }
%  \title{Beyond Linear Bias SGD: Reshuffling meets Richardson: }
%  \title{When Reshuffling Meets Extrapolation:\\Sharper Bias in Constant Step-Size SGD}
  \title{Shuffling the Data, Stretching the Step-Size:\\Sharper Bias  in Constant Step-Size SGD}
 
%	•	Debiasing Stochastic Gradient Methods: The Synergy of Reshuffling and Richardson Extrapolation
%	•	From $\mathcal{O}(\gamma)$ to $\mathcal{O}(\gamma^3)$: Bias Reduction in Constant Step-Size Stochastic Optimization

==> gamma-neighbors.tex <==
% !TEX root = ./iclr2026_conference.tex

\tikzset{every picture/.style={line width=0.75pt}}        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]


%Shape: Ellipse [id:dp7329906304802944] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.29 ] (481.22,393.5) .. controls (481.22,299.89) and (557.06,224) .. (650.61,224) .. controls (744.16,224) and (820,299.89) .. (820,393.5) .. controls (820,487.11) and (744.16,563) .. (650.61,563) .. controls (557.06,563) and (481.22,487.11) .. (481.22,393.5) -- cycle ;
%Shape: Ellipse [id:dp14673386188875415] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.41 ] (537.7,393.5) .. controls (537.7,331.1) and (588.25,280.52) .. (650.61,280.52) .. controls (712.97,280.52) and (763.52,331.1) .. (763.52,393.5) .. controls (763.52,455.9) and (712.97,506.48) .. (650.61,506.48) .. controls (588.25,506.48) and (537.7,455.9) .. (537.7,393.5) -- cycle ;
%Shape: Ellipse [id:dp3138874134344609] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (568.79,393.5) .. controls (568.79,348.28) and (605.42,311.62) .. (650.61,311.62) .. controls (695.8,311.62) and (732.44,348.28) .. (732.44,393.5) .. controls (732.44,438.72) and (695.8,475.38) .. (650.61,475.38) .. controls (605.42,475.38) and (568.79,438.72) .. (568.79,393.5) -- cycle ;
%Shape: Ellipse [id:dp6951380714624634] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.73 ] (617.47,393.5) .. controls (617.47,375.18) and (632.31,360.34) .. (650.61,360.34) .. controls (668.91,360.34) and (683.75,375.18) .. (683.75,393.5) .. controls (683.75,411.82) and (668.91,426.66) .. (650.61,426.66) .. controls (632.31,426.66) and (617.47,411.82) .. (617.47,393.5) -- cycle ;

% =============== COLORED POLYLINES WITH STARS ===============

% Green path
\draw [color={rgb, 255:red, 110; green, 192; blue, 19 }, line width=2.25]
  (356,490) -- (341,370) -- (418,243) -- (508,191) -- (594,212) -- (626.22,296.33);
\foreach \p in {(356,490),(341,370),(418,243),(508,191),(594,212),(626.22,296.33)}{
  \node[star, star points=5, draw={rgb,255:red,110; green,192; blue,19},
        fill={rgb,255:red,110; green,192; blue,19}, minimum size=7pt, inner sep=0pt] at \p {};
}

% Blue path
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }, line width=2.25]
  (356,490) -- (321,336) -- (362,258) -- (424,199) -- (499,157) -- (607,151)
  -- (698,178) -- (728,218) -- (713.68,258.29);
\foreach \p in {  (356,490) , (321,336) , (362,258) , (424,199) , (499,157) , (607,151)
  , (698,178) , (728,218) , (713.68,258.29)}{
  \node[star, star points=5, draw={rgb,255:red,74; green,144; blue,226},
        fill={rgb,255:red,74; green,144; blue,226}, minimum size=7pt, inner sep=0pt] at \p {};
}

% Orange path
\draw [color={rgb, 255:red, 206; green, 131; blue, 13 }, line width=2.25]
  (356,490) -- (388,387) -- (498,266) -- (574,267) -- (601,279) -- (618.6,339.2);
\foreach \p in {(356,490),(388,387),(498,266),(574,267),(601,279),(618.6,339.2)}{
  \node[star, star points=5, draw={rgb,255:red,206; green,131; blue,13},
        fill={rgb,255:red,206; green,131; blue,13}, minimum size=7pt, inner sep=0pt] at \p {};
}

% Red path
\draw [color={rgb, 255:red, 165; green, 6; blue, 24 }, line width=2.25]
  (356,490) -- (420,388) -- (504,346) -- (580,343) -- (641.61,376.61);
\foreach \p in {(356,490),(420,388),(504,346),(580,343),(641.61,376.61)}{
  \node[star, star points=5, draw={rgb,255:red,165; green,6; blue,24},
        fill={rgb,255:red,165; green,6; blue,24}, minimum size=7pt, inner sep=0pt] at \p {};
}

% =============================================================
%
%% Text Node
%\draw (632.38,393.8) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ]  {$x_{*}$};
%% Text Node
%\draw (606.03,200.22) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,rotate=-0.45]  {$\mathrm{bias}( \gamma ) =\ \mathcal{O}\left( \gamma \right)$};
%% Text Node
%\draw (671.93,254.71) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 100; green, 172; blue, 43 },opacity=1 ,rotate=-25.81]  {$\mathrm{bias}( \gamma ) =\ \mathcal{O}\left( \gamma ^{1.5}\right)$};
%% Text Node
%\draw (598.56,429.08) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ,rotate=-0.61]  {$\mathrm{bias}( \gamma ) =\ \mathcal{O}\left( \gamma ^{3}\right)$};
%% Text Node
%\draw (720.43,309.21) node [anchor=north west][inner sep=0.75pt]  [font=\large,color={rgb, 255:red, 231; green, 151; blue, 19 }  ,opacity=1 ,rotate=-60.58]  {$\mathrm{bias}( \gamma ) =\ \mathcal{O}\left( \gamma ^{2}\right)$};
%% Text Node
%\draw (372.38,478.8) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$x_{0}$};

% Text Node
\draw (632.38,393.8) node [anchor=north west][inner sep=0.75pt]  [font=\Large,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ]  {$x_{*}$};
% Text Node
\draw (606.03,200.22) node [anchor=north west][inner sep=0.75pt]  [font=\large,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,rotate=-0.45]  {$\mathrm{bias}( \gamma ) =\ O( \gamma )$};
% Text Node
\draw (665.93,244.71) node [anchor=north west][inner sep=0.75pt]  [font=\large,color={rgb, 255:red, 83; green, 146; blue, 2 }  ,opacity=1 ,rotate=-25.81]  {$\mathrm{bias}( \gamma ) =\ O\left( \gamma ^{1.5}\right)$};
% Text Node
\draw (595.56,429.08) node [anchor=north west][inner sep=0.75pt]  [font=\large,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ,rotate=-0.61]  {$\mathrm{bias}( \gamma ) =\ O\left( \gamma ^{3}\right)$};
% Text Node
\draw (716.43,301.21) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize,color={rgb, 255:red, 180; green, 117; blue, 0 }  ,opacity=1 ,rotate=-60.58]  {$\mathrm{bias}( \gamma ) =\ O\left( \gamma ^{2}\right)$};
% Text Node
\draw (365.38,478.8) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$x_{0}$};

%Straight Lines [id:da7873343135782715] 
\draw    (650.61,393.5) -- (648.05,234) ;
\draw [shift={(648,231)}, rotate = 89.08] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
\draw [shift={(650.61,393.5)}, rotate = 269.08] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da8747548930371518] 
\draw    (650.61,393.5) -- (695.72,297.71) ;
\draw [shift={(697,295)}, rotate = 115.22] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
\draw [shift={(650.61,393.5)}, rotate = 295.22] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da18150789044644122] 
\draw    (650.61,393.5) -- (713.61,347.16) ;
\draw [shift={(716.03,345.38)}, rotate = 143.66] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
\draw [shift={(650.61,393.5)}, rotate = 323.66] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da6863210759512379] 
\draw    (650.61,393.5) -- (665.12,418.22) ;
\draw [shift={(666.64,420.81)}, rotate = 239.59] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
\draw [shift={(650.61,393.5)}, rotate = 59.59] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;



% % Central point and labels
% \draw (632.38,393.8) node [anchor=north west][inner sep=0.75pt] [font=\large,color=white] {$x_{*}$};
% \draw (606.03,200.22) node [anchor=north west][font=\footnotesize,color={rgb, 255:red, 74; green, 144; blue, 226 }] {$\mathrm{bias}( \gamma ) =\ O( \gamma )$};
% \draw (671.93,254.71) node [anchor=north west][font=\footnotesize,color={rgb, 255:red, 126; green, 211; blue, 33 }] {$\mathrm{bias}( \gamma ) =\ O\!\left( \gamma ^{1.5}\right)$};
% \draw (598.56,429.08) node [anchor=north west][font=\footnotesize,color={rgb, 255:red, 208; green, 2; blue, 27 }] {$\mathrm{bias}( \gamma ) =\ O\!\left( \gamma ^{3}\right)$};
% \draw (720.43,309.21) node [anchor=north west][font=\footnotesize,color={rgb, 255:red, 231; green, 151; blue, 19 }] {$\mathrm{bias}( \gamma ) =\ O\!\left( \gamma ^{2}\right)$};
% \draw (372.38,478.8) node [anchor=north west][font=\large,color=black] {$x_{0}$};

\end{tikzpicture}

==> rr_intuition_figure.tex <==
% rr_intuition_figure.tex — v14
\begin{tikzpicture}[
    >=stealth,
    every node/.style={font=\small},
    dot/.style={circle,fill,inner sep=2.8pt},
    lbl/.style={inner sep=6pt, rounded corners=4pt, thick},
]
  \colorlet{colA}{blue!75!black}
  \colorlet{colB}{orange!85!black}
  \colorlet{colR}{red!60!black}
  \definecolor{darkgreen}{RGB}{80,160,10}

  \def\yB{4.20}
  \def\yA{2.00}
  \def\yMid{3.10}
  \def\yE{0.00}
  \def\xT{8.0}
  \def\xRul{9.2}

  % ── Asymptote dashed lines ───────────────────────────────────────
  \draw[colB, densely dashed, opacity=0.40, thin] (0,\yB) -- (\xRul+0.3,\yB);
  \draw[colA, densely dashed, opacity=0.40, thin] (0,\yA) -- (\xRul+0.3,\yA);
  \draw[gray!30, densely dashed, thin] (0,\yE) -- (\xRul+5.5,\yE)
    node[right, gray!45, font=\small] {$x^*$};

  % ── Funnels: manually defined polygons that CONTAIN the trajectories
  \fill[colB, opacity=0.10]
    (0,6.15) .. controls (2,5.52) and (4,4.92) .. (6,4.63) -- (\xT,4.48)
    -- (\xT,3.92) -- (6,4.07) .. controls (4,4.18) and (2,4.28) .. (0,4.85)
    -- cycle;

  \fill[colA, opacity=0.12]
    (0,-0.05) .. controls (2,1.45) and (4,1.85) .. (6,1.92) -- (\xT,2.22)
    -- (\xT,1.78) -- (6,1.48) .. controls (4,0.95) and (2,0.15) .. (0,-1.35)
    -- cycle;

  % ── Trajectories ─────────────────────────────────────────────────
  \draw[colA, line width=1.9pt, ->]
    plot[smooth,tension=0.55] coordinates
      {(0,-0.7)(2,0.8)(4,1.4)(6,1.7)(\xT,\yA)};
  \draw[colB, line width=1.9pt, ->]
    plot[smooth,tension=0.55] coordinates
      {(0,5.5)(2,4.9)(4,4.55)(6,4.35)(\xT,\yB)};

  % ── Faint sphere halos (before dots) ─────────────────────────────
  \node[circle, fill=colB, fill opacity=0.13, draw=colB, draw opacity=0.22,
        inner sep=22pt] at (\xT,\yB) {};
  \node[circle, fill=colA, fill opacity=0.13, draw=colA, draw opacity=0.22,
        inner sep=22pt] at (\xT,\yA) {};
  \node[circle, fill=black, fill opacity=0.10, draw=black, draw opacity=0.18,
        inner sep=11pt] at (\xT+1.3,\yMid) {};

  % ── Terminal dots ────────────────────────────────────────────────
  \node[dot,colA] (zA) at (\xT,\yA) {};
  \node[dot,colB] (zB) at (\xT,\yB) {};
  \node[colA, left=12pt, font=\small\itshape] at (zA) {$x^{k+2}_{\gamma}$};
  \node[colB, left=12pt, font=\small\itshape] at (zB) {$x^{k+2}_{2\gamma}$};

  % ── Extrapolated dot ─────────────────────────────────────────────
  \node[dot,black,inner sep=2.8pt] (xhat) at (\xT+1.3,\yMid) {};
  \node[black, above=5pt, font=\small\bfseries] at (xhat) {$\hat{x}^{k+2}$};

  % ── Run labels ───────────────────────────────────────────────────
  \node[colA, draw=colA, fill=blue!5, lbl] at (1.8,-1.70)
    {\textbf{Run A}\enspace(step $\gamma$)};
  \node[colB, draw=colB, fill=orange!5, lbl] at (1.8, 6.4)
    {\textbf{Run B}\enspace(step $2\gamma$)};

  % ── Bias annotation boxes (inside plot) ──────────────────────────
  \node[colA, draw=colA, fill=blue!4, lbl] at (4.2, 0.45)
    {$\mathrm{Bias}=A\cdot\gamma+\mathcal{O}(\gamma^3)$};
  \node[colB, draw=colB, fill=orange!4, lbl] at (4.2, 5.60)
    {$\mathrm{Bias}=A\cdot(2\gamma)+\mathcal{O}(\gamma^3)$};

  % ── Epoch k ──────────────────────────────────────────────────────
  \draw[->, darkgreen, line width=1.5pt]
    (-0.2,-2.30) -- (\xT+0.3,-2.30);
  \node[darkgreen, right=5pt, font=\small\bfseries]
    at (\xT+0.3,-2.30) {Epoch $k$};

\end{tikzpicture}
